Estimating the Density Ratio between Distributions with High Discrepancy using Multinomial Logistic Regression

Functions of the ratio of the densities $p/q$ are widely used in machine learning to quantify the discrepancy between the two distributions $p$ and $q$. For high-dimensional distributions, binary classification-based density ratio estimators have shown great promise. However, when densities are well separated, estimating the density ratio with a binary classifier is challenging. In this work, we show that the state-of-the-art density ratio estimators perform poorly on well-separated cases and demonstrate that this is due to distribution shifts between training and evaluation time. We present an alternative method that leverages multi-class classification for density ratio estimation and does not suffer from distribution shift issues. The method uses a set of auxiliary densities $\{m_k\}_{k=1}^K$ and trains a multi-class logistic regression to classify the samples from $p, q$, and $\{m_k\}_{k=1}^K$ into $K+2$ classes. We show that if these auxiliary densities are constructed such that they overlap with $p$ and $q$, then a multi-class logistic regression allows for estimating $\log p/q$ on the domain of any of the $K+2$ distributions and resolves the distribution shift problems of the current state-of-the-art methods. We compare our method to state-of-the-art density ratio estimators on both synthetic and real datasets and demonstrate its superior performance on the tasks of density ratio estimation, mutual information estimation, and representation learning. Code: https://www.blackswhan.com/mdre/

==> s1-intro-old.tex <==
\section{Introduction}
\label{sec:intro}
Quantification of the discrepancy between two distributions underpins a large number of machine learning techniques.
For instance, distribution discrepancy measures known as $f$-divergences \citep{csiszar1964}, which are defined as expectations of the functions of the ratio of two densities, are ubiquitous in many domains of machine learning. Hence, density ratio estimation is often a central task in generative modeling, mutual information and divergence estimation, and representation learning \citep{sugiyama2012density,nce,gan,fgan,veegan,belghazi2018mine,infonce,gram}. However, estimating the density ratio by modeling each of the densities separately is challenging for most problems of interest. 
% as modeling high dimensional densities is a harder problem than estimating their ratios 
\cite{sugiyama2012density}.

% it either requires a closed-form expression of the densities or analytical expressions of density ratios are hard to derive for most problems of interest, as it requires knowledge of the functional form of the underlying densities.
% Therefore, in practice, density ratio estimators are employed that only require samples from the pair of densities instead of modeling them individually.
Therefore, in practice, direct density ratio estimation, rather than separate modeling of the individual densities and taking the ratio, is employed,
% to provide an estimate of the density ratio directly
usually given samples from the pair of densities only.
One of the most commonly used density ratio estimators (DRE) utilizes binary classification via logistic regression (BC-DRE), which estimates the ground truth density ratio when trained to discriminate between the samples from the two densities \citep[e.g.][]{nce, Gutmann2011b, sugiyama2012density,menon2016linking}.
% \looseness=-1

BC-DREs have been tremendously successful in problems involving the minimization of the discrepancy between the data and the model distributions even in high-dimensional settings \citep{fgan,dcgan}. However, they do not fare as well when applied to the task of estimating the discrepancy between two distributions that are far apart or easily separable otherwise. This issue has been characterized recently as the \emph{density-chasm problem} by \citet{tre}. The discrepancy between two distributions can manifest itself in many different ways. We roughly categorize them into two classes: \emph{First Order Discrepancy (FOD)} and \emph{Higher Order Discrepancy (HOD)}. Two distributions can be easily separated when the first order statistics, such as their means(or an affine transformation of the mean), are far apart from each other. We refer to this type of discrepancy between $p$ and $q$ as FOD. Similarly, if the discrepancy between $p$ and $q$ (with no FOD) originates due to the difference in second or higher order moments, we refer to this as HOD. For example, consider Figure \ref{fig:hod_fod}, where in all the three cases, the $\text{KL}[p\Vert q] = 50$, but in (a) it originates from FOD since $\mathcal{N}(\mu_1=-5, \sigma_1=1)$ and $\mathcal{N}(\mu_1=5, \sigma_1=1)$ differ only in means, in (b) it originates from HOD since $\mathcal{N}(\mu_1=0, \sigma_1=1)$ and $\mathcal{N}(\mu_2=0, \sigma_1=0.097)$ differ only in variances, and in (c) it originates from FOD and HOD since $\mathcal{N}(\mu_1=-1.5, \sigma_1=0.5)$ and $\mathcal{N}(\mu_2=1, \sigma_1=0.25)$ differ in both means and variances.
% \looseness=-1

% In a recent work, \cite{choi2021featurized} attempt to address the density-chasm problem. They considered distributions $p$ and $q$ that are clearly separated and proposed that in such cases density ratios can be better estimated if the mixture of the two densities is mapped onto a unit-sphere using a flow-based map \citep{rezende2015variational}. Using a bijective map ensures that the density ratio between the original distributions is maintained post mapping. While this method (F-DRE) may resolve the density-chasm problem due to FOD, we found that it struggles when the densities are separated due to HOD.

% On the other hand, \cite{tre} proposed to estimate the density ratio between $p$ and $q$ as $\frac{p}{p_1}\times \frac{p_1}{p_2} \times \dots \times \frac{p_K}{q}$. This telescoping is achieved by training $K$ BC-DREs where the distributions $p_1, \dots , p_k$ are designed to be \emph{closely-packed} such that all of the $K$ ratios can be easily estimated using BC-DREs without suffering from the density-chasm problem. They call this estimator, telescoping density ratio estimator or TRE. Empirically, we found that while TRE performs relatively better than BC-DRE and F-DRE in cases with density-chasm problem due to HOD, it cannot deal with the density-chasm problem originating due to FOD. Intuitively, this happens because TRE trains $K$ DREs, each of which is trained on $K$ different pairs of distributions. This leads to the distribution shift issue at test time, especially when $p$ and $q$ have high FOD. Further, care needs to be taken when designing intermediate distributions $p_1, \dots ,p_K$ to ensure that each of the ratios are well defined. In fact, the construction schemes introduced in the original work may render TRE theoretically ill-defined if both $p$ and $q$ do not have full support (Appendix \ref{app:constructing_m}).
Recent works have tried to address the density-chasm problem. However, we found that these state-of-the-art methods are only capable of solving problems with either high FOD \cite{choi2021featurized} or high HOD \cite{tre}. As such, to the best of our knowledge, no single method addresses density ratio estimation problems that involve both FOD and HOD at the same time. However, most problems in practice tend to have both types of discrepancies. This leaves a clear technical gap in the task of density ratio estimation. 

% \begin{wrapfigure}{r}{0.23\textwidth}
\begin{figure}
% \vspace{-1em}
\centering
\includegraphics[width=0.25\textwidth]{fig/1d/fod_hod.png}
\caption{\small First Order vs Higher Order Discrepancies.\label{fig:hod_fod}}
% \vspace{-1em}
% \end{wrapfigure}
\end{figure}

We present \COB (\cob), a novel method for density ratio estimation that can deal with the density-chasm issues arising from both high FOD and HOD.
The intuition behind \cob is to replace the \textit{easy} binary classification problem that suffers from the density-chasm issue when $p$ and $q$ are well separated with a \textit{harder} multi-class classification problem. To this end, \cob first constructs a set of $K$ auxiliary distributions $\{m_k\}_{k=1}^K$ that overlap with $p$ and $q$ and then trains a multi-class logistic regression on the $K+2$ distributions to obtain a density ratio estimator of $\log p/q$. 
Following are the key contributions of this work:
\begin{enumerate}
    \item We study the existing solutions to the density chasm issue and identify their limitations that has not been previously explored.
    \item We show that the state-of-the-art solution to the density chasm issue \cite{tre} can lead to distribution shift or out-of distribution evaluation issues, which in turns significantly degrades ratio estimation.
    \item We prove that cross-entropy-based training of multinomial logistic regression leads to a multi-distribution density ratio estimator and then show that it does not suffer from the aforementioned distribution-shift issue. 
    \item We conduct a very detailed empirical evaluation of the proposed approach and demonstrate the superior performance of our method on a number of benchmarks. Our results show that \cob is often an order of magnitude better than the current state-of-the-art of density ratio estimation tasks such as mutual-information estimation. 
\end{enumerate}
% The use of the auxiliary distributions is similar to the approach by \citet{tre}. But, we leverage the auxiliary distributions in a different manner: we solve a single multi-class classification problem, while \citet{tre} solve a sequence of binary classification problems. Importantly, we show that their approach can lead to distribution shift or out-of distribution evaluation issues, which our approach avoids.
%Further, we identify a distribution shift issue in the most recent method on resolving density-chasm \cite{tre} and show that \cob resolves this distribution shift by construction.
% We show that our method is theoretically well-defined and while the current state-of-art method \cite{tre} suffers from a distribution shift issues, \cob does not.
% Our simulations demonstrate that \cob significantly outperforms the state-of-the-art on the tasks of density ratio estimation, mutual information estimation, and representation learning while being computationally more efficient.

==> s2-back-old.tex <==
\section{Notation and Background}
\label{sec:notation}
% Bregman distance between two $d$-dimensional vectors $a$ and $b$ is defined as $D_f(a,b) = f(a) - f(b) - \nabla f(b)(a-b)$, where $f:\mathbb{R}^d \mapsto \mathbb{R}$ is a convex function.
% Following the notation in \citet{StummerV12}, scaled Bregman Divergence (sBD) between probability measures $P$ and $Q$ scaled by some measure $M$ can be defined as
% \begin{align}\label{eq:scaledBreg}
% &D_{f}(P,Q |M) \\=& \int_{\cal X} m \Bigg [f\left(\frac{p}{m}\right) - f \left(\frac{q}{m}\right) - f'\left(\frac{q}{m}\right) \left(\frac{p}{m} - \frac{q}{m} \right) \Bigg ]d \lambda, \nonumber
% \end{align}
% where $f: \mathcal{X}\rightarrow \mathbb{R}$ is a convex function and $f'$ is its right-hand derivative. Further, all the measures $P,Q$ and $M$ are defined on the measurable space $(\mathcal{X},\mathcal{A})$ and are absolutely continuous with respect to a $\sigma$-finite measure $\lambda$, therefore admitting the following densities,
% \begin{align}
% \label{eq:densities}
%     p = \frac{dP}{d\lambda} ,\quad q = \frac{dQ}{d\lambda} ,\quad m = \frac{dM}{d\lambda}.
% \end{align}


Let $P$ and $Q$ be probability measures defined on some measurable space $(\mathcal{X},\mathcal{A})$ such that they are absolutely continuous with respect to a $\sigma$-finite measure $\lambda$, therefore admitting the following densities, $p = \frac{dP}{d\lambda} ,\quad q = \frac{dQ}{d\lambda}$.

Given samples $\{x_p^i\}_{i=1}^N$ and $\{x_q^j\}_{j=1}^M$ from distributions $p$ and $q$ respectively and assuming that $p$ is absolutely continuous with respect to $q$ i.e. $p << q$, the goal in density ratio estimation is to construct an estimator $\hat r_{p/q}$ of $p/q$.

% \subsection{Binary Classification to DRE using BD}
% Proposition 3 of \citet{menon2016linking} formally establishes the link between binary classification and density ratio estimation using sBD, which we rephrase in Proposition~\ref{prop:multi-class}.
% \begin{proposition}[Proposition 3, \citet{menon2016linking}]
% \label{prop:multi-class}
% Given a class-probability estimator $\hat \eta: \mathcal{X} \mapsto [0,1]$ such that the density ratio estimator, $\hat r_{p/q}(x) = \frac{\hat \eta}{1-\hat \eta}.$
% % \begin{align}
% %     \hat r_{p/q}(x) = \frac{\hat \eta}{1-\hat \eta}.
% % \end{align}
% Then for any convex differentiable function $f: [0,1] \mapsto \mathbb{R}$,
% \begin{align}\label{eq:prop3}
%     &\mathbb{E}_{x \sim p_\text{x}} [D_f(\eta(X) \Vert \hat \eta(X)] \\=& \frac{1}{2}\mathbb{E}_{x \sim q}[D_{f^\dagger} (r_{p/q}(X)\Vert\hat r_{p/q}(X))] \nonumber
% \end{align}
% where $D_f$ is Bregman Divergence (BD), $f^\dagger: [0,\infty) \mapsto \mathbb{R} \;\vert\; f^\dagger(x) = (1+x)f(\frac{x}{1+x})$,  $\mathbb{E}_{x\sim q}[D_{f^\dagger}]$ is sBD and $p_{\text{x}}=0.5 \times p(x) + 0.5 \times q(x) $ is the distribution of $X$.
% \end{proposition}

\subsection{Density Chasm} 
\citet{kato2021non} note that most DREs, especially those implemented with a deep neural network, tend to over-fit the loss function to the training data in some way or the other. Relatedly, \citet{tre} showed that BC-DREs can solve the corresponding classification problem nearly perfectly if the distributions $p$ and $q$ are very different, but still yield poor estimates of the ratio $p/q$. They termed the difficulty of estimating the ratio of highly different distributions the "density-chasm problem".
%This phenomenon was recently characterized by \citet{tre} for the BC-DRE as the density-chasm problem. They found that, despite poorly estimating the ratio $p/q$, BC-DREs can solve the corresponding classification problem nearly perfectly if the distributions $p$ and $q$ are very different. 
We conjecture that this underestimation occurs due to high epistemic uncertainty. That is, in finite data setting, when the two sets of samples are easily separable, many different decision boundaries are possible that correspond to similar low empirical Bayes risk, but are far from the Bayes optimal classifier in the asymptotic regime.

As a consequence of the poor estimation of the density ratio, BC-DREs also tend to typically substantially underestimate the ground-truth Kullback-Leibler (KL) divergence when computed with the estimated ratio. This underestimation stems from the \textit{sigmoid} link function, $\sigma(t) = \frac{1}{1+e^{-t}}$, that is commonly used in logistic regression to convert the logit that represents the log-ratio ($\log p(x)/q(x)$), into the class probability. Since this link function saturates at values of log-ratio that are higher than 6, which, one the classes are well-separable, allows to reach high accuracy, leads to underestimation of the log-ratio. In order to verify our hypothesis, we show in Figure [TODO], that when trained with non-gradient based learning method such as Metropolis-Hastings, while logistic regression still provides a bad estimation of the log-ratio, it does however overestimates it.

==> s3-related-old.tex <==
\section{Related Work}
\label{sec:related_work}
\begin{figure}[ht!]
        \centering
        \begin{subfigure}[b]{.95\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/1d/1D_demo_tre_K=3_from_logpq.png}
            \caption[]%
            {{\small TRE 3 waymarks.}}
            \label{fig:tre_insight}
        \end{subfigure}
        
        \begin{subfigure}[b]{.95\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/1d/1D_demo_cob_K=1_cauchy_logpq.png}
            \caption[]
            {\small \cob with $m=\cauchydist(0,1)$}
            \label{fig:1dcobdemo}
        \end{subfigure}
        
        \begin{subfigure}[b]{.95\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/1d/1D_demo_cob_K=3_logpq.png}
            \includegraphics[width=\textwidth]{fig/1d/1D_cob_trewm_pm_qm.png}
            \caption[]
            {{\small \cob using TRE waymarks as scaling measures.}}
            \label{fig:cob_insight_2}
        \end{subfigure}
        % % \vskip\baselineskip
        \caption[]
        {\small TRE vs \cob on estimation of $\log$ density ratio where $p=\mathcal{N}(-1,0.1)$ and $q=\mathcal{N}(1,0.2)$. 
        % Please see Appendix \ref{app:trevscob}, Figure \ref{fig:app_trevscob} for higher-resolution version. 
        }
        \label{fig:trevscob}
        \vspace{-1em}
    \end{figure}
    
In this section, we describe two density ratio estimation methods, \citet{tre} and \citet{choi2021featurized}, which represent the current state-of-the-art on solving the density-chasm problem.

% Our work is closely related to and improves upon the shortcomings of the recently proposed TRE method that only reduces the density-chasm problem issues due to high HOD. 
% Therefore, in order to better understand these shortcomings, we begin by analyzing TRE under Proposition 3 of \cite{menon2016linking} as described in \eqref{eq:prop3} above. 
Telescoping Density Ratio Estimator or TRE \citep{tre} uses a two step, divide-and-conquer strategy to tackle the density-chasm problem. In the first step, they construct $K$ \emph{waymark} distributions $p_1, \dots , p_K$ by \emph{gradually} transporting samples from $p$ towards samples from $q$. Then, they train $K$ BC-DREs, one for each consecutive pairs of distributions. This allows for estimating the ratio $r_{p/q}$ as the product of the $K+1$ BC-DREs, $r_{p/q} := \frac{p}{q} = \frac{p}{p_1} \times \dots \times \frac{p_K}{q}$. 
They introduced two schemes for creating waymark distributions that ensure that consecutive pairs of distributions are packed \emph{closely enough} so that none of the $K+1$ BC-DREs suffers from the density-chasm issue. Hence, TRE addresses the density-chasm issue by replacing the ratio between $p$ and $q$ with a product of $K+1$ intermediate density ratios that by design of the waymark distribution should not suffer from the density-chasm problem. In a new work, \citet{choi2021density} introduced $\text{DRE-}\infty$, where they took the number of waymark distributions in TRE to infinity and derived a limiting objective that leads to a more scalable version of TRE.\looseness=-1

\textbf{Distribution Shift in TRE:}
In supervised learning, distribution shift \cite{quinonero2009dataset} occurs when the training data $(x,y) \sim p_{\text{train}}$ and the test data $(x,y)\sim p_{\text{test}}$ come from two different
distributions i.e. $p_{\text{train}} \neq p_{\text{test}}$. This leads the classifier to be biased to the training data which severely degrades its performance on the test data.

We now show that a similar distribution shift occurs in the TRE model especially when distributions $p$ and $q$ have high FOD.
Let the BC-DREs corresponding to the $K+1$ density ratios $p/p_1, \dots, p_K/q$ in TRE be $\hat \eta_1, \dots, \hat \eta_{K+1}$. Given the theoretical properties of BC-DRE, for any $i \in \{1,\dots,K+1\}$, $\hat \eta_i$ upon training should accurately estimate $r_{p_{i-1}/p_i}$ on the support of $p_i$ (Proposition 3 of \citet{menon2016linking}, \cite{nce}). However, when evaluating the ratio $p/q$, the individual $\hat \eta_i$ are evaluated on the support of $q$ (which is equal or larger than the support of $p$) while trained on data from the support of $p_i$. When the FOD is high, however, there is barely an overlap between $p_i, p$ and $q$ as shown in the first panel of Figure \ref{fig:tre_insight}. Hence, we evaluate each density ratio model $\hat \eta_i$ on inputs far away from the training data and, therefore, each density ratio model suffers from distribution shift problems.  
% This holds true for samples from all the other $K$ distribution that are significantly different from the training distributions $p_{i-1}$ and $p_i$ of $\hat \eta_i$. 
This shift in the distribution at evaluation time causes significant degradation in TRE's performance as we empirically demonstrate in later sections.
\looseness=-1
% causes significant degradation in performance.   
% Application of Proposition \ref{prop:multi-class} to TRE shows that each of the individual binary classifiers, upon training lead to $K+1$ DREs that minimize the sBD to their corresponding true density ratios on the samples from their corresponding denominator densities.
% This however, does not guarantee that a product of such individual DREs minimizes the sBD to $r_{p/q}$ on samples from $q$ (or all $K$ intermediate distributions for $K>1$). 
% as equation \eqref{eq:prop3} cannot be applied to the product of independently trained density ratio estimators. 
% This is because the optimality of individual estimator to convergence to the true density ratio is only guaranteed under the expectation from their corresponding denominator densities. 
% is acknowledged by the authors who note that TRE's performance suffers significantly when the distributions $p$ and $q$ have high FOD. 

An example of this can be seen in Figure \ref{fig:tre_insight} where we train TRE to estimate the density ratio between $p=\mathcal{N}(-1,0.1)$ and $q=\mathcal{N}(+1,0.2)$, which is ratio estimation problem with significant FOD. We use 3 intermediate distributions $p_1, p_2, p_3$ constructed with the \textit{linear-mixing} construction described in Section \ref{sec:constructing_m}. In the first row, we evaluate the ratios $p/p_1, p_1/p_2, p_2/p_3$ and $p_3/q$ on samples from their respective denominator densities and in the second row we evaluate $\log \frac{p}{q}$ on samples from all the $K+2$ distributions. We see that individual DREs accurately estimate their corresponding density ratios on  their corresponding training distributions. But, the telescoping does not lead to an accurate estimation of $p/q$ for samples from any of the $K+2$ distributions except $p_2$. This renders TRE less useful for estimating discrepancy measures, such as KL divergence, as the model is not accurate on the domain of $p$, especially when there is high FOD. Further, we found that despite estimating the $\frac{p}{q}$ accurately, TRE's waymark construction schemes can render the some intermediate ratios $\frac{m}{q}$ theoretically ill-defined during training when both $p$ and $q$ do not have full support; see Appendix \ref{app:trevscob} for a detailed discussion.
% \paragraph{Distributions with finite support: }
% \label{sec:constructing_m}
% \cite{tre} proposed two schemes for constructing intermediate distributions $p_k$ for TRE; linear mixing and dimension-wise mixing. However, both of these construction schemes may lead to theoretical inconsistencies when the distributions $p$ and $q$ only have finite support. We demonstrate this issue with an example in Section \ref{sec:vstre}.

% Let $\mathcal{TN}$ stand for truncated Normal distribution and consider the following setup: \\
% $p = 0.5 \times \mathcal{TN}(-1, 0.1, low=-1.1, high=-0.9) + 0.5 \times \mathcal{TN}(1, 0.1, low=0.9, high=1.1)$, \\
% $q = 0.5 \times \mathcal{TN}(-1, 0.2, low=-1.2, high=0.8) + 0.5 \times \mathcal{TN}(1, 0.2, low=0.8, high=1)$ \\
% %$m = \mathcal{TN}(0, 1, low=-1.2, high=1.2)$. 
% In this case, if $p_k$ is constructed using their construction schemes, it is no longer true that $p_k<<q$ as samples from $p_k$ will fall out of the support of $q$ (See Appendix [TODO] for details). Therefore, the ratio $m/q$ is not defined, rendering the entire chain of telescoping estimators undefined.

% \paragraph{F-DRE: }
Another interesting related work comes from \citet{choi2021featurized} (F-DRE). They employ a FLOW-based model \cite{rezende2015variational} on the input and train it to map the samples from the mixture of the  two distributions to a standard Gaussian and then train a BC-DRE. It is easy to show that any bijective map will preserve the original density ratio $r_{p/q}$ in the feature space as the Jacobian correction term simply cancels out. However, such a method cannot \textit{bring the distributions closer} in terms of both FOD and HOD. This is because, in order for a FLOW to maintain the original density ratio, reducing FOD increases HOD and vice-versa such that the net discrepancy between $p$ and $q$ remains unchanged. Due to this issue, in practice, we found that F-DRE works only in fairly limited settings. 

Finally, \citet{liu2021analyzing} recently introduced an optimization-based solution to the density-chasm problem in exponential family distributions by using (a) normalized gradient descent and (b) replacing the logistic loss with the exponential loss.

==> s4-mrdre-old.tex <==
\section{Density Ratio Estimation using Multinominal Logistic Regression}
% \section{Density Ratio Estimation by Scaling Densities}

We propose \COB (\cob) to tackle the density-chasm problems by leveraging auxiliary distributions through multinominal logistic regression.
In \cob, we introduce a set of $K$ auxiliary distributions $\{m_k\}_{k=1}^K$ and formulate the problem of estimating $\log \frac{p}{q}$ as a multi-class classification problem.
% To this end, in \cob, we first scale the densities $p$ and $q$ by one (or more) probability measure(s) $m$ and estimate $\log \frac{p}{q}$ as $\log \frac{p}{m} - \log \frac{q}{m}$. 
%We show in the next section that if the measures $\{m_k\}_{k=1}^K$ are constructed such that $\forall{k}, p<<m_k, q<<m_k$ , then a single multi-class logistic regression trained to classify samples from $p, q$ and $\{m_i\}_{k=1}^M$ into $K+2$ classes, can be used to estimate $\log p/q$ as the difference of their corresponding un-normalized log probabilities (\eqref{eq:estimator}). This estimator remains accurate on the domain of all $K+2$ distributions and hence avoids the distribution shift issue. \looseness=-1
We show in the next section that a single multi-class logistic regression trained to classify samples from $p, q$ and $\{m_k\}_{k=1}^M$ into $K+2$ classes, can be used to estimate $\log p/q$ as the difference of their corresponding un-normalized log probabilities (\eqref{eq:rhat-def}). This estimator is accurate on the domain of all $K+2$ distributions and hence resolves the distribution shift issue.
\looseness=-1


\subsection{Multinomial Logistic Regression to Multi-distribution DRE}
We first establish that, for a probabilistic classifier with softmax activation, the difference in logit space between two classes can be used to estimate the (log) density ratio between the corresponding distributions.

Consider a parametric probabilistic classifier with categorical likelihood function, that models the probability of sample $x \sim p_x$ belonging to the component distribution $p_c$ as, $P(Y=c|x; \theta)= \frac{\pi_c\exp(h^c_\theta(x))}{\sum_{k=1}^C\pi_k\exp(h^k_\theta(x))}$, where $h_\theta^c$ refers to the logit corresponding to the $c^\text{th}$ class, i.e.~the unnormalized log probabilities.
Upon maximum likelihood training, the following estimate can be used to represent the log-density ratio $\log {p_i(x) \over p_j(x)}$
$$
\hat r_{p_i / p_j}(x) := h_\theta^i(x) - h_\theta^j(x).
$$
We summarize this claim as Proposition~\ref{prop:cob} and show its proof.

\begin{proposition}[\cob estimate]
Let $p_x(x) = \sum_{c=1}^C \pi_c p_c(x)$ be the mixture of the $C$ distributions $\{p_c\}_{c=1}^C$ where the $c^{\text{th}}$ entry ($\pi_c$) of the $C$-dimensional vector $\pi$ denotes the mixing coefficient for distribution $p_c$. Then, given a parametric probabilistic classifier with categorical likelihood function, that models the probability of sample $x \sim p_x$ belonging to the component distribution $p_c$ as, $P(Y=c|x; \theta)= \frac{\pi_c\exp(h^c_\theta(x))}{\sum_{k=1}^C\pi_k\exp(h^k_\theta(x))}$, the density ratio between $p_i$ and $p_j$ for any $i,j \leq C$ is given by
\begin{align}
    \label{eq:estimator}
    \log\frac{p_i(x)}{p_j(x)} = h_\theta^i(x)-h_\theta^j(x).
\end{align}
\label{prop:cob}
\end{proposition}
where $h_\theta^c$ refers to the logit corresponding to the $c^\text{th}$ class, i.e.~the unnormalized log probabilities, 
upon maximum likelihood training on samples from $p_x$, i.e. $\theta = \theta^\ast$
\begin{equation}
    \theta^\ast = \argmin_{\theta} \mathcal{L}(\theta)= \argmax_{\theta} \sum_{c=1}^C \pi_c \mathbb{E}_{x\sim p_c}[\log P(Y=c|x; \theta)]. 
\end{equation}

\begin{proof}
% Let $p_x(x) = \sum_{c=1}^C \pi_c p_c(x)$ be the mixture of the $C$ distributions $\{p_c\}_{c=1}^C$ where the $c^{\text{th}}$ entry ($\pi_c$) of the $C$-dimensional vector $\pi$ denotes the mixing coefficient for distribution $p_c$. Then the multi-class classification problem consists of predicting the correct class $Y \in\{1, \ldots, C\}$ given a sample from the mixture $p_x$. The probability of a sample $x$ belonging to mixture component $p_c$ is then given by 
% \begin{align*}
%     P(Y=c|x; \theta)= \frac{\pi_c\exp(h^c_\theta(x))}{\sum_{k=1}^C\pi_k\exp(h^k_\theta(x))},
% \end{align*}
Since $\theta$ admits a categorical likelihood, we can estimate it by minimizing the softmax cross-entropy loss (negative log-loss) $\mathcal{L}(\theta)$,
\begin{align}
\label{eq:multinomial-loss}
    \mathcal{L}(\theta)&= - \sum_{c=1}^C \pi_c \mathbb{E}_{x\sim p_c}[\log P(Y=c|x; \theta)]. 
\end{align}
We denote the optimal parameters by $\optmodel = \argmin_\theta \mathcal{L}(\theta)$.
% We now show that for flexible enough functions $h^c_\theta(x)$, minimizing the above loss functions allows us to estimate the log ratios between any pairs of the mixing distributions $p_c$, which we exploit to estimate $r_{p/q}$. 
For flexible parametrizations, we can consider the above loss function as a functional of $C$ functions $h_1,\dots , h_C$ and for brevity, we denote $h^c_\theta(x)$ as $h_c$ in the following.,
\begin{align}
    \mathcal{L}(h_1,\dots , h_C) &=\sum_{c=1}^C \pi_c \mathbb{E}_{x\sim p_c}\bigg[-\log \pi_c - h_c(x) +\log \sum_{k=1}^C \pi_k\exp(h_k(x)) \bigg].
\end{align}
Using $p_x=\sum_{c=1}^C\pi_cp_c$ on the second and the third term inside the expectation, we have
\begin{align}
    \mathcal{L}(h_1,\dots , h_C)&=\sum_{c=1}^C \pi_c \mathbb{E}_{x\sim p_c}[-\log \pi_c - h_c(x)] + \int p_x(x) [\log \sum_{k=1}^C \pi_k\exp(h_k(x)) ]dx. \nonumber
\end{align}
The functional derivative of $\mathcal{L}(h_1,\dots , h_C)$ with respect to $h_i$ equals
\begin{align}
\label{eq:partial}
    \frac{\partial \mathcal{L}}{\partial h_i} = \pi_ip_i(x) - p_x(x)\frac{\pi_i\exp(h_i(x))}{\sum_{k=1}^C\pi_k\exp(h_k(x))}
\end{align}
for all $x$ where $p_x(x)>0$. Setting $\frac{\partial L}{\partial h_i}$ to zero, we thus have
\begin{align}
\label{eq:critical}
    \frac{\pi_ip_i(x)}{p_x(x)} = \frac{\pi_i\exp(h_i(x))}{\sum_{k=1}^C\pi_k\exp(h_k(x))};\quad i=1,\dots, C .
\end{align}
The left-hand side of \eqref{eq:critical} is the true class conditional, $P^*(Y=i|x) = \frac{\pi_ip_i(x)}{p_x(x)}$. Hence, at the critical point, $h_1,\dots,h_C$ are such that $P^*(Y|X)$ is correctly estimated. From \eqref{eq:critical}, it follows that for two arbitrary $i$ and $j$, we have $\frac{\pi_ip_i}{\pi_jp_j}=\frac{\pi_i\exp(h_i)}{\pi_j\exp(h_i)}$ i.e
\begin{align}
    \label{eq:estimator}
    \log\frac{p_i(x)}{p_j(x)} = h_i(x)-h_j(x).
\end{align}
\end{proof}
This key property of the multinomial loss function in \eqref{eq:multinomial-loss} allows to estimate $r_{p/q}$ by formulating the ratio estimation problem as a multinomial nonlinear regression problem with $p_1 \equiv p, p_2 \equiv q, p_3, \equiv m_1, \ldots, p_{K+2} \equiv m_K$ and setting
\begin{equation}
\label{eq:rhat-def}
\hat{r}_{p/q}(x) = h^1_{\optmodel}(x)-h^2_{\optmodel}(x).    
\end{equation}
Since \eqref{eq:critical} holds for all $x$ where the mixture $p_x(x)>0$, our estimator $\hat{r}_{p/q}(x)$ is valid for all $x$ in the union of the domain of $p, q, m_1, \ldots, m_K$. Please note, in practice, we use a uniform prior over the classes i.e. $\pi_c=1/(K+2)$.

\begin{proposition}[Identifiability]
\end{proposition}
While we have $C$ unknowns $h_1,\dots,h_C$ and $C$ equations, there is a redundancy in the equations because summing \eqref{eq:critical} overall $i$ gives $\sum_{i=1}^C\frac{\pi_ip_i(x)}{p_x(x)} = \sum_{i=1}^C \frac{\pi_c\exp(h_c(x))}{\sum_{k=1}^C\pi_k\exp(h_k(x)}=1$. This means that we cannot uniquely identify all $h_i$. This is true for \textit{softmax logistic-regression} in general. However, the difference $h_i-h_j$ of the logits, for any $i$ and $j$, can be identified and equals to the desired log ratio between $p_i$ and $p_j$ per \eqref{eq:estimator}. 

% \paragraph{Cosnsistency:}   Softmax logistic regression, when parameterized using the difference of logits, is not only identifiable but also reduces to multinomial logit model and can be expressed as $C-1$ independent binary logistic regression models. Let $h_C$ be the logit corresponding to an arbitrarily chosen pivot class, assuming uniform prior over the classes and subtracting $h_C$ from the argument of the exponentials in \eqref{eq:critical} we have,
% \begin{align}
% \label{eq:con1}
%     P(Y=i|x) = \frac{\exp(h_i(x)-h_C(x))}{1+\sum_{k=1}^{C-1}\exp(h_k(x)-h_C(x))}; \quad i=1,\dots, C .
% \end{align}
% That is, for the difference of the logit parameterization, the softmax logisitic regression is equivalent to $C-1$ independent logistic regressions, which are consistent estimators of the true density ratio as shown by \cite{nce}. Since each of the $K-1$ DREs are consistent, thus their differences (MR-DRE), $h_i-h_j$ is also consistent.

% Consider a set of $C$ distributions $\{p_c\}_{c=1}^C$ and let $p_x(x) = \sum_{c=1}^C \pi_c p_c(x)$ be their mixture distribution. Here, the $c^{\text{th}}$ entry ($\pi_c$) of the $C$-dimensional vector $\pi$ denotes the mixing coefficient for component $p_c$. The multi-class classification problem now consists of predicting the correct class $Y \in\{1, \ldots, C\}$ from a sample from the mixture $p_x$. For this purpose, we consider the model 
% \begin{align*}
%     P(Y=c|x; \theta)= \frac{\pi_c\exp(h^c_\theta(x))}{\sum_{k=1}^C\pi_k\exp(h^k_\theta(x))},
% \end{align*}
% where the $h^c_\theta(x)$, $c=1, \ldots, C$ are unnormalized log probabilities parametrized by $\theta$. We estimate $\theta$ by minimizing the softmax cross-entropy loss (negative log-loss) $\mathcal{L}(\theta)$,
% \begin{align}
% \label{eq:multinomial-loss}
%     \mathcal{L}(\theta)&= - \sum_{c=1}^C \pi_c \mathbb{E}_{x\sim p_c}[\log P(Y=c|x; \theta)]. 
% \end{align}
% We denote the optimal parameters by $\optmodel = \argmin_\theta \mathcal{L}(\theta)$.

% \textbf{Estimating $r_{p/q}$: } We now show that for flexible enough functions $h^c_\theta(x)$, minimizing the above loss functions allows us to estimate the log ratios between any pairs of the mixing distributions $p_c$, which we exploit to estimate $r_{p/q}$. For brevity, we denote $h^c_\theta(x)$ as $h_c$ in the following.

% % Let a discrete random variable $Y$ be the class label. For notational clarity, let the log-scores $h^c_\optmodel$ for class $C$ be denoted by $h_c$. Then,
% % \begin{align*}
% %     P(Y=c|x)= \frac{\pi_c\exp(h_c(x))}{\sum_{k=1}^C\pi_k\exp(h_k(x)}.
% % \end{align*}
% For flexible parametrizations, we can consider the above loss function as a function of $C$ functions $h_1,\dots , h_C$,
% \begin{align}
%     \mathcal{L}(h_1,\dots , h_C) &=\sum_{c=1}^C \pi_c \mathbb{E}_{x\sim p_c}\bigg[-\log \pi_c - h_c(x) \nonumber \\ &\quad \quad +\log \sum_{k=1}^C \pi_k\exp(h_k(x)) \bigg].
% \end{align}
% Using $p_x=\sum_{c=1}^C\pi_cp_c$ on the second term, we have
% \begin{align}
%     \mathcal{L}(h_1,\dots , h_C)&=\sum_{c=1}^C \pi_c \mathbb{E}_{x\sim p_c}[-\log \pi_c - h_c(x)] \\ &\quad + \int p_x(x) [\log \sum_{k=1}^C \pi_k\exp(h_k(x)) ]dx. \nonumber
% \end{align}
% The functional derivative of $\mathcal{L}(h_1,\dots , h_C)$ with respect to $h_i$ equals
% \begin{align}
% \label{eq:partial}
%     \frac{\partial L}{\partial h_i} = \pi_ip_i(x) - p_x(x)\frac{\pi_i\exp(h_i(x))}{\sum_{k=1}^C\pi_k\exp(h_k(x))}
% \end{align}
% for all $x$ where $p_x(x)>0$. Setting $\frac{\partial L}{\partial h_i}$ to zero, we thus have
% \begin{align}
% \label{eq:critical}
%     \frac{\pi_ip_i(x)}{p_x(x)} = \frac{\pi_i\exp(h_i(x))}{\sum_{k=1}^C\pi_k\exp(h_k(x))};\quad i=1,\dots, C .
% \end{align}
% The left-hand side of \eqref{eq:critical} is the true class conditional, $P^*(Y=i|x) = \frac{\pi_ip_i(x)}{p_x(x)}$. Hence, at the critical point, $h_1,\dots,h_C$ are such that $P^*(Y|X)$ is correctly estimated. Further, while we have $C$ unknowns $h_1,\dots,h_C$ and $C$ equations, there is a redundancy in the equations because summing \eqref{eq:critical} over all $i$ gives $\sum_{i=1}^C\frac{\pi_ip_i(x)}{p_x(x)} = \sum_{i=1}^C \frac{\pi_c\exp(h_c(x))}{\sum_{k=1}^C\pi_k\exp(h_k(x)}=1$. This means that we cannot uniquely identify all $h_i$. However, their difference $h_i-h_j$ for any $i$ and $j$ can be identified and equals to the desired log ratio between $p_i$ and $p_j$: From \eqref{eq:critical}, it follows that for two arbitrary $i$ and $j$, we have $\frac{\pi_ip_i}{\pi_jp_j}=\frac{\pi_i\exp(h_i)}{\pi_j\exp(h_i)}$ i.e
% \begin{align}
%     \label{eq:estimator}
%     \log\frac{p_i(x)}{p_j(x)} = h_i(x)-h_j(x).
% \end{align}
% This key property of the multinomial loss function in \eqref{eq:multinomial-loss} allows to estimate $r_{p/q}$ by formulating the ratio estimation problem as a multinomial nonlinear regression problem with $p_1 \equiv p, p_2 \equiv q, p_3, \equiv m_1, \ldots, p_{K+2} \equiv m_K$ and setting
% \begin{equation}
% \label{eq:rhat-def}
% \hat{r}_{p/q}(x) = h^1_{\optmodel}(x)-h^2_{\optmodel}(x).    
% \end{equation}
% Since \eqref{eq:critical} holds for all $x$ where the mixture $p_x(x)>0$, our estimator $\hat{r}_{p/q}(x)$ is valid for all $x$ in the union of the domain of $p, q, m_1, \ldots, m_K$. Please note, in practice we use a uniform prior over the classes i.e. $\pi_c=1/(K+2)$.


\subsection{Distribution Shift Free}
Since the multi-class classifier of \cob is trained on the mixture of $K+2$ distributions, that is, $p_{\text{train}} = \frac{1}{K+2} (p+q+\sum_{k=1}^Km_k)$ and valid on its whole domain, it does not suffer from any distribution shift issues when evaluated on samples from any of the $K+2$ distributions. As such, it performs drastically better than other methods on tasks such as $f$-divergence and mutual information estimation where \cob is evaluated on data that comes from one of the $K=2$ training distributions. 

% distribution $p_{\text{test}}$ for evaluation is the same as the training distribution i.e  $p_{\text{train}} = \frac{1}{K+2} (p+q+\sum_{k=1}^Km_k) = p_{\text{test}}$.

% As such it performs drastically better than other methods on tasks such as  as for these tasks the distribution $p_{\text{test}}$ of the evaluation data le.

% As such, for tasks, such as $f$-divergence and mutual information estimation, that require evaluation on samples from one of the $K+2$ distributions, \cob performs drastically better.

We demonstrate this in Figure \ref{fig:1dcobdemo} and Figure \ref{fig:cob_insight_2}. Here, we train \cob with exactly the same problem setup as TRE in Figure \ref{fig:tre_insight} where $p=\mathcal{N}(-1,0.1)$ and $q=\mathcal{N}(1,0.2)$. In Figure \ref{fig:1dcobdemo}, we propose to use $\cauchydist(0,1)$ as the auxiliary measure. This is because the samples from the heavy tailed distributions overlap with the highly concentrated samples of $p$ and $q$ as shown in Figure \ref{fig:1dcobdemo}. Then we train a single 3-way logistic regression to classify samples from $p, q$ and $m$. We can clearly see that \cob is able to estimate $\log p/q$ well on samples from all the three distributions without suffering from any distribution shift issues. 

To demonstrate that the improved performance of \cob over TRE in the example from Figure \ref{fig:trevscob} does not only stem from the choice of $m$ (see section \ref{sec:constructing_m}), we also train \cob using TRE's waymark distributions as auxiliary measures. This is illustrated in Figure \ref{fig:cob_insight_2} (top row). Unlike TRE that does not estimate $\log \frac{p}{q}$ accurately on samples from $p, p_1, p_3$, and $q$, \cob is able to estimate $\log \frac{p}{q}$ on all 5 distributions significantly better even with the sub-optimal choice of auxiliary measures. Further, in Figure \ref{fig:cob_insight_2} (bottom row), we show that \cob also accurately estimates $p/m_k$ and $q/m_k$ on the support of $m_k$ for all $K$ auxiliary measures. Please see Appendix \ref{app:trevscob} for the full scale version of these plots and other details.
\looseness=-1

While TRE turns an easy binary classification problem into a sequence of harder binary classification problems, \cob turns the same easy binary classification problem into a harder multi-class classification problem. For TRE, the original problem is the composition of the new problems, while for \cob, the original problem is a “sub-problem” of the new one and thus avoids distribution shift.

It is worth pointing out that while here we relate a multinomial logistic regression to DRE, other class-probability estimators, in the multi-class setting, may also be related to density ratio estimation \cite{nock2016scaled}.

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=\textwidth]{fig/1d/mu--1_2_inoutdomain.pdf}
        \caption{$p=\mathcal{N}(-1, 0.08), q=\mathcal{N}(2, 0.15)$}
        \label{fig:1d_ratios_-1_2_inoutdom}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=\textwidth]{fig/1d/mu--2_2_inoutdomain.pdf}
        \caption{$p=\mathcal{N}(-2, 0.08), q=\mathcal{N}(2, 0.15)$}
        \label{fig:1d_ratios_-2_2_inoutdom}
    \end{subfigure}
    \caption{\small Mean and 1 standard deviation of the log-ratio estimates on in-domain and expanded-domain on the configurations in Table \ref{1dtask}. Note that the ground truth and \cob curves are overlapping. } \label{fig:1d_ratios_plot} 
\end{figure*}

\subsection{Constructing the Auxiliary Measures}
\label{sec:constructing_m}
In this work, we use three ways of constructing the auxiliary measures. Here, we describe them briefly. Please see Appendix \ref{app:constructing_m} for details.
\textbf{Overlapping Distribution: }
We introduce a novel auxiliary measure construction scheme under which, $m_k$ is defined as any distribution whose samples overlap with both $p$ and $q$ and $p << m_k$, $q << m_k$. For example, it can be heavy-tailed distributions, such as Cauchy and Student-t, or simply normal and uniform distributions or their mixtures.
\textbf{Linear Mixing: }
In this construction scheme, distribution $m_k$ is defined as the empirical distribution of the samples constructed by linearly combining samples $X_p = \{x_p^i\}_{i=1}^N$ and $X_q = \{x_q^i\}_{i=1}^N$ from distributions $p$ and $q$ respectively. That is, $m_k$ is the empirical distribution over the set $X_{m_k} = \{x_{m_k}^i | x_{m_k}^i = (1-\alpha_k) x_p^i + \alpha_k x_q^i, x_p \in X_p, x_q^i \in X_q \}_{i=1}^N$, where $0 < \alpha_k < 1$. This construction is related to the linear combination waymark of \citet{tre}. We clarify the difference in Appendix \ref{app:constructing_m}.
% The main difference is that \cob linear mixing is a simple convex combination of the samples from $p$ and $q$ that does not use the skewed weighting from TRE. This allows for samples from $m$ to have higher variance and overlap with the samples of both $p$ and $q$\\
\textbf{Dimension-wise Mixing: }In this construction scheme, which is borrowed from TRE \citep{tre} as it is, $m$ is defined as the empirical distribution of the samples generated by combining different subsets of dimensions from samples from $p$ and $q$. 
